Toward Resource-Optimal Consensus over the Wireless Medium

We carry out a comprehensive study of the resource cost of averaging consensus in wireless networks. Most previous approaches suppose a graphical network, which abstracts away crucial features of the wireless medium, and measure resource consumption only in terms of the total number of transmissions required to achieve consensus. Under a path-loss dominated model, we study the resource requirements of consensus with respect to three wireless-appropriate metrics: total transmit energy, elapsed time, and time-bandwidth product. First we characterize the performance of several popular gossip algorithms, showing that they may be order-optimal with respect to transmit energy but are strictly suboptimal with respect to elapsed time and time-bandwidth product. Further, we propose a new consensus scheme, termed hierarchical averaging, and show that it is nearly order-optimal with respect to all three metrics. Finally, we examine the effects of quantization, showing that hierarchical averaging provides a nearly order-optimal tradeoff between resource consumption and quantization error.

==> jsac/simulations.2.tikz.tex <==
% !TEX root = ../jsac.tex

\begin{tikzpicture}
			
	\begin{scope}[scale=1]
	\begin{loglogaxis}[
	%title={$P=20$dB},
	xlabel={$N$},
	ylabel={Total Transmit Energy},
	%axis x line=bottom,
	%axis y line=left,
	%height=125pt,
	%width=250pt,
	legend style={at={(0.65,2.21)}},
	]
		
		\addplot[thick,mark=x,mark options=solid,dotted,green] file {jsac/randomE.2.data};
		\addlegendentry{\small Randomized };
		
		\addplot[very thick,mark=triangle,mark options=solid,dotted,red] file {jsac/pathAveragingE.2.data};
		\addlegendentry{\small Path Averaging};
		
		%\addplot[color=green!50!black, thick,dashed] file {jsac/multiscaleE.data};
		%\addlegendentry{\small Multi-scale };
		
		\addplot[very thick,mark=star,mark options=solid,dashed,purple] file {jsac/cHierarchicalE.2.data};
		\addlegendentry{\small Hierarchical Averaging};
		
		%\addplot[very thick, mark=square,mark options=solid,dashed,purple] file {jsac/cHierarchicalE.data};
		%\addlegendentry{\small Hierarchical  (fixed phase)};
		
		\addplot[very thick,mark=o,orange] file {jsac/lowerBoundE.2.data};
		\addlegendentry{\small Lower Bound };

	\end{loglogaxis}
	\end{scope}
	
	\begin{scope}[scale=1,yshift=200]
	\begin{loglogaxis}[
	%title={$P=20$dB},
	xlabel={$N$},
	ylabel={Time-bandwidth Product},
	ymax=5000000,
	%axis x line=bottom,
	%axis y line=left,
	%height=125pt,
	%width=250pt,
	%legend style={font=\Large,text=black},
	]

		\addplot[thick,mark=x,mark options=solid,dotted,green]  file {jsac/randomD.2.data};
		%\addlegendentry{\small Randomized };
		
		\addplot[very thick,mark=triangle,mark options=solid,dotted,red] file {jsac/pathAveragingD.2.data};
		%\addlegendentry{\small Path Averaging};
		
		%\addplot[color=green!50!black, thick,dashed] file {jsac/multiscaleD.data};
		%\addlegendentry{\small Multi-scale };
		
		\addplot[very thick,mark=star,mark options=solid,dashed,purple] file {jsac/cHierarchicalD.2.data};
		%\addlegendentry{\small Hierarchical  (uniform phase)};
		
		%\addplot[very thick, mark=square,mark options=solid,dashed,purple] file {jsac/cHierarchicalD.data};
		%\addlegendentry{\small Hierarchical  (fixed phase)};
		\addplot[very thick,orange,domain=10:1000] {1};

	\end{loglogaxis}
	\end{scope}
\end{tikzpicture}

==> jsac/simulations.alpha.tikz.tex <==
% !TEX root = reviewer.response.tex

\begin{tikzpicture}
			
	\begin{scope}[scale=0.9]
	\begin{semilogyaxis}[
	%title={$P=20$dB},
	xlabel={$\alpha$},
	ylabel={Total Transmit Energy (J)},
	%axis x line=bottom,
	%axis y line=left,
	%height=125pt,
	%width=250pt,
	legend pos = {outer north east}
	]
		
		\addplot[thick,mark=x,mark options=solid,dotted,green] file {randomE.alpha.data};
		\addlegendentry{\small Randomized Gossip};
		
		\addplot[very thick,mark=triangle,mark options=solid,dotted,red] file {pathAveragingE.alpha.data};
		\addlegendentry{\small Path Averaging};
		
		%\addplot[color=green!50!black, thick,dashed] file {jsac/multiscaleE.data};
		%\addlegendentry{\small Multi-scale };
		
		\addplot[very thick,mark=star,mark options=solid,dashed,blue] file {hierarchicalE.alpha.data};
		\addlegendentry{\small Hierarchical (uniform phase)};
		
		\addplot[very thick, mark=square,mark options=solid,dashed,purple] file {cHierarchicalE.alpha.data};
		\addlegendentry{\small Hierarchical (fixed phase)};
		
		\addplot[very thick,mark=o,orange] file {lowerBoundE.alpha.data};
		\addlegendentry{\small Lower Bound };

	\end{semilogyaxis}
	\end{scope}
	
	\begin{scope}[scale=0.9,yshift=-200]
	\begin{semilogyaxis}[
	%title={$P=20$dB},
	xlabel={$\alpha$},
	ylabel={Time-bandwidth Product},
	%ymax=500000000,
	%axis x line=bottom,
	%axis y line=left,
	%height=125pt,
	%width=250pt,
	%legend style={font=\Large,text=black},
	]

		\addplot[thick,mark=x,mark options=solid,dotted,green]  file {randomD.alpha.data};
		%\addlegendentry{\small Randomized };
		
		\addplot[very thick,mark=triangle,mark options=solid,dotted,red] file {pathAveragingD.alpha.data};
		%\addlegendentry{\small Path Averaging};
		
		%\addplot[color=green!50!black, thick,dashed] file {jsac/multiscaleD.data};
		%\addlegendentry{\small Multi-scale };
		
		\addplot[very thick,mark=star,mark options=solid,dashed,blue] file {hierarchicalD.alpha.data};
		%\addlegendentry{\small Hierarchical  (uniform phase)};
		
		\addplot[very thick, mark=square,mark options=solid,dashed,purple] file {cHierarchicalD.alpha.data};
		%\addlegendentry{\small Hierarchical  (fixed phase)};

	\end{semilogyaxis}
	\end{scope}
\end{tikzpicture}
